Oblivious RAM Simulation with Efficient Worst-Case Access Overhead

Oblivious RAM simulation is a method for achieving confidentiality and privacy in cloud computing environments. It involves obscuring the access patterns to a remote storage so that the manager of that storage cannot infer information about its contents. Existing solutions typically involve small amortized overheads for achieving this goal, but nevertheless involve potentially huge variations in access times, depending on when they occur. In this paper, we show how to de-amortize oblivious RAM simulations, so that each access takes a worst-case bounded amount of time.

==> conclusion.tex <==
\section{Conclusion}
We have presented methods for oblivious RAM simulation with efficient
worst-case access overhead.  Our methods are based on de-amortizing two
known solutions, the square root approach and the $\log n$ hierarchical
approach, which have efficient amortized access overhead but $\Omega(n)$
access overhead in the worst case.
%
For each of our methods,
the worst-case access overhead per request is asymptotically equal to the
amortized access overhead of the solution it is based on.  In
particular, our $\log n$ hierarchical solution incurs $\log n$ access
overhead on every request.
%


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> related_work.tex <==
\section{Related Work}


